Simplified vine copula models: state of science and affairs

Vine copula models have become highly popular practical tools for modeling multivariate dependencies. To maintain tractability, a commonly employed simplifying assumption is that conditional copulas remain unchanged by the conditioning variables. This assumption has sparked a somewhat polarizing debate within the copula community. The fact that much of this dispute occurs outside the public record has placed the field in an unfortunate position, impeding scientific progress. In this article, I will review what we know about the flexibility and limitations of simplified vine copula models, explore the broader implications, and offer my own, hopefully reconciling, perspective on the issue.

==> latex-templates/theorems.tex <==
\usepackage{shadethm}
\usepackage{etoolbox}

% theorem environments

\newtheoremstyle{new}
  {12pt}      % Space above
  {12pt}      % Space below
  {\itshape}  % Body font
  {}          % Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries\color{LMUgreen}} % head font
  {.}         % Punctuation after  head
  { }         % Space after  head: " " = normal inter-word space; \newline = line break
  {}          % head spec (can be left empty, meaning 'normal')
\theoremstyle{new}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Korollar}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Annahme}
\newtheorem{example}[theorem]{Beispiel}
\newtheorem{remark}[theorem]{Anmerkung}

\AfterEndEnvironment{theorem}{\noindent\ignorespaces}
\AfterEndEnvironment{corollary}{\noindent\ignorespaces}
\AfterEndEnvironment{proposition}{\noindent\ignorespaces}
\AfterEndEnvironment{lemma}{\noindent\ignorespaces}
\AfterEndEnvironment{definition}{\noindent\ignorespaces}
\AfterEndEnvironment{assumption}{\noindent\ignorespaces}
\AfterEndEnvironment{example}{\noindent\ignorespaces}
\AfterEndEnvironment{remark}{\noindent\ignorespaces}

\Crefname{theorem}{Theorem}{Theoreme}
\Crefname{corollary}{Korollar}{Korollare}
\Crefname{proposition}{Proposition}{Propositionen}
\Crefname{lemma}{Lemma}{Lemmas}
\Crefname{definition}{Definition}{Definitionen}
\Crefname{example}{Beispiel}{Beispiele}
\Crefname{remark}{Anmerkung}{Anmerkungen}

\usepackage[breakable, theorems, skins]{tcolorbox}
\tcbset{enhanced}

% same environments with shaded background
\definecolor{shadethmcolor}{cmyk}{0,0,0,0.075}    
% \definecolor{shadethmcolor}{cmyk}{0.5, 0, 0.425, 0.075}    
\definecolor{shaderulecolor}{rgb}{1,1,1}   % color of frame 

\DeclareRobustCommand{\mybox}[1]{%
\begin{tcolorbox}[   %% Adjust the following parameters at will.
        breakable,
        left=0pt,
        right=0pt,
        top=0pt,
        bottom=0pt,
        colback=shadethmcolor,
        colframe=shaderulecolor,
        width=\dimexpr\textwidth\relax, 
        enlarge left by=0mm,
        boxsep=5pt,
        arc=0pt,outer arc=0pt,
        ]
        #1
\end{tcolorbox}
}

\setlength{\shadeboxrule}{1.2pt}   % width of frame
\setlength{\shadeboxsep}{7pt}
\setlength\shadedtextwidth{\dimexpr\textwidth-2\shadeboxsep\relax}
\newtheoremstyle{shad}
  {12pt}      % Space above
  {12pt}      % Space below
  {\itshape }  % Body font
  {}          % Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries\color{LMUgreen}} % head font
  {.}         % Punctuation after head
  { }         % Space after head: " " = normal inter-word space; \newline = line break
  {}          % head spec (can be left empty, meaning 'normal')
\theoremstyle{shad} 

\newshadetheorem{thmbox}[theorem]{Theorem}
\newshadetheorem{corbox}[theorem]{Korollar}
\newshadetheorem{propbox}[theorem]{Proposition}
\newshadetheorem{lembox}[theorem]{Lemma}
\newshadetheorem{exbox}[theorem]{Beispiel}
\newshadetheorem{defbox}[theorem]{Definition}
\newshadetheorem{rembox}[theorem]{Anmerkung}

\newtheoremstyle{shad*}
  {12pt}      % Space above
  {12pt}      % Space below
  {\itshape }  % Body font
  {}          % Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries\color{LMUgreen}} % head font
  {.}         % Punctuation after head
  { }         % Space after head: " " = normal inter-word space; \newline = line break
  {}          % head spec (can be left empty, meaning 'normal')
\theoremstyle{shad*} 
\newshadetheorem{anobox}{}

\Crefname{theorem}{Theorem}{Theoreme}
\Crefname{corbox}{Korollar}{Korollare}
\Crefname{propbox}{Proposition}{Propositionen}
\Crefname{lembox}{Lemma}{Lemmas}
\Crefname{exbox}{Beispiel}{Beispiele}
\Crefname{defbox}{Definition}{Definitionen}
\Crefname{rembox}{Anmerkung}{Anmerkungen}

